Defending Text-to-image Diffusion Models: Surprising Efficacy of Textual Perturbations Against Backdoor Attacks

Text-to-image diffusion models have been widely adopted in real-world applications due to their ability to generate realistic images from textual descriptions. However, recent studies have shown that these methods are vulnerable to backdoor attacks. Despite the significant threat posed by backdoor attacks on text-to-image diffusion models, countermeasures remain under-explored. In this paper, we address this research gap by demonstrating that state-of-the-art backdoor attacks against text-to-image diffusion models can be effectively mitigated by a surprisingly simple defense strategy - textual perturbation. Experiments show that textual perturbations are effective in defending against state-of-the-art backdoor attacks with minimal sacrifice to generation quality. We analyze the efficacy of textual perturbation from two angles: text embedding space and cross-attention maps. They further explain how backdoor attacks have compromised text-to-image diffusion models, providing insights for studying future attack and defense strategies. Our code is available at https://github.com/oscarchew/t2i-backdoor-defense.

==> tables/training_configs_TI.tex <==
\begin{tabular}{lcl}
    \toprule
    Argument & Value & Meaning\\
    \midrule
    \texttt{max\_train\_steps} & $2000$ & Maximum number of training steps.\\
    \texttt{effective training\_batch\_size} & $4$ & Batch size for training.\\
    \texttt{placeholder\_token} & \textbf{trigger} & The special token representing the object.\\
    % \texttt{initializer\_token} & \textbf{concept} & A single-word describes the object. \\
    \bottomrule
\end{tabular}
